Faithful-First Reasoning, Planning, and Acting for Multimodal LLMs

Multimodal Large Language Models (MLLMs) frequently suffer from unfaithfulness, generating reasoning chains that drift from visual evidence or contradict final predictions. We propose Faithful-First Reasoning, Planning, and Acting (RPA) framework in which FaithEvi provides step-wise and chain-level supervision by evaluating the faithfulness of intermediate reasoning, and FaithAct uses these signals to plan and execute faithfulness-aware actions during inference. Experiments across multiple multimodal reasoning benchmarks show that faithful-first RPA improves perceptual faithfulness by up to 24% over prompt-based and tool-augmented reasoning frameworks, without degrading task accuracy. Our analysis shows that treating faithfulness as a guiding principle perceptually faithful reasoning trajectories and mitigates hallucination behavior. This work thereby establishes a unified framework for both evaluating and enforcing faithfulness in multimodal reasoning. Code is at https://github.com/lijunxian111/Faithful-First-RPA.

==> sec/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

==> sec/experiments.tex <==
\section{Experiments}
The purpose of this Section is to illustrate the better performance of our planner on faithfulness of the reasoning chain, as well as good performance on correctness. We'll also include further experiments on ablation, distribution of $F_{step_{i}}$, etc. All results are reported in percentage (\%).

\begin{table*}[t]
    \small
    \centering
    \begin{tabular}{r|ccc}
    \toprule
       Datasets \& Models  & \textbf{LLaVA-bench (\%)} & \textbf{RealWorldQA (\%)} & \textbf{MMHal (\%)} \\
       \midrule
        Qwen-2.5-VL-7B~\cite{Bai2025Qwen25VLTR}+CoT & 46.05$\pm$19.58 & 48.11$\pm$27.04 & 53.34$\pm$24.02\\
        +ReAct & \underline{54.82$\pm$26.53} & \underline{56.82$\pm$31.71} & 33.76$\pm$28.43 \\
        +Grounded-CoT & 50.04$\pm$17.54 & 53.35$\pm$26.68 & \underline{56.77$\pm$25.86} \\
        +VAT & 51.59$\pm$21.37 & 50.13$\pm$26.43 & 55.32$\pm$28.58 \\
        +\textbf{FaithAct (ours)} & \textbf{55.10$\pm$20.14} & \textbf{57.22$\pm$27.85} & \textbf{66.45$\pm$27.87}\\
        \midrule
        InternVL3-8B~\cite{Zhu2025InternVL3EA}+CoT & 45.63$\pm$16.60 & 44.23$\pm$25.43 & 53.17$\pm$23.64 \\
        +ReAct & \textbf{51.97$\pm$24.08} &  \underline{56.56$\pm$31.30} & 31.61$\pm$29.61 \\
        +Grounded-CoT & 48.35$\pm$18.05 & 47.94$\pm$19.36 & 18.10$\pm$14.96 \\
        +VAT & 48.97$\pm$17.22 & 45.31$\pm$28.19 & \underline{54.51$\pm$26.99} \\
        +\textbf{FaithAct (ours)} & \underline{51.85$\pm$18.66} & \textbf{57.35$\pm$29.40} & \textbf{61.71$\pm$27.01}\\
        \midrule 
         LLaVA-one-Vision-1.5-8B~\cite{an2025llavaonevision15fullyopenframework}+CoT & 47.56$\pm$23.35 & 52.31$\pm$28.44 & 30.63$\pm$28.56 \\
        +ReAct & \textbf{59.20$\pm$27.18} & \underline{56.82$\pm$31.71} & \underline{32.23$\pm$31.73} \\
        +Grounded-CoT & 50.62$\pm$18.74 & 52.30$\pm$28.89 & 31.69$\pm$27.00 \\
        +VAT  & 46.16$\pm$19.46 & 50.15$\pm$30.66 & 30.30$\pm$28.96 \\
        +\textbf{FaithAct (ours)} & \underline{52.82$\pm$22.77} & 
        \textbf{58.11$\pm$30.37} & \textbf{39.91$\pm$27.92}\\
        \bottomrule
    \end{tabular}
    \caption{Faithfulness evaluation results (with or without our planner). We report mean and standard deviation of $F_{chain}$ here by percentage (\%). The best performance is \textbf{highlighted} and second best is \underline{underlined}.}
    \label{tab:faith_eval}
\end{table*}

\begin{table*}[t]
    \centering
    \begin{tabular}{l|ccc}
    \toprule
       Datasets \& Models  & \textbf{LLaVA-bench (\%)} & \textbf{RealWorldQA (\%)} & \textbf{MMHal (\%)} \\
       \midrule
        Qwen-2.5-VL-7B~\cite{Bai2025Qwen25VLTR}+CoT & 100.0 & 70.1 & 75.8 \\
        
        +\textbf{FaithAct (ours)} & 100.0 & 74.5 & 76.8 \\
        \bottomrule
    \end{tabular}
    \caption{\label{tab:correctness}Correctness when applying FaithAct on Qwen-2.5-VL-7B.}
\end{table*}

\noindent \textbf{Datasets.} We select several real-world multimodal benchmarks like LLaVA-bench~\cite{Liu2023VisualIT}, RealWorldQA~\cite{xai_grok1_5} and MMHal-Bench~\cite{2023llavarlhf} (MMHal). The images in these benchmarks usually contain lots of real-world objects, and it's convenient for faithfulness evaluation on them.

\noindent \textbf{Models.} We choose several widely-used MLLMs for our task. Qwen-2.5-VL-7B~\cite{Bai2025Qwen25VLTR}, InternVL3-8B~\cite{Zhu2025InternVL3EA} and LLaVA-one-Vision-1.5-8B~\cite{an2025llavaonevision15fullyopenframework} are chosen.

\noindent \textbf{Baselines.} We compare our method with several reasoning methods that do not training the MLLM itself. CoT~\cite{wei2022chain, zhang2023multimodal} is utilized as a baseline for simply generating reasoning chains, We also apply ReAct~\cite{yao2022react}, Grounded-CoT~\cite{Wu2025GroundedCF}, and Visual Abstract Thinking (VAT)~\cite{liu2025visual} for reasoning with the help of extra object information. ReAct enables MLLMs to automatically call useful functions during reasoning (we provide the same functions for it as our FaithAct's). While Grounded-Cot requires MLLMs to ground the objects in reasoning by itself during reasoning, and VAT provide MLLMs abstract images (sketch, etc.) together with the original image to benefit from multi-level information.

\noindent \textbf{Generation Hyper-parameters.} The box\_threshold of GroundingDINO is 0.35 and the text\_threshold is 0.25. We keep the default generation settings for helper LLM and MLLMs.


\subsection{Main Results and Findings}
Table~\ref{tab:faith_eval} shows the performance of FaithAct compared with selected baseline methods. The experimental results highlight several key findings. 

\noindent \textbf{Faithfulness is Underestimated.} First, while faithfulness remains a challenge across all models, the overall scores indicate that further improvements are needed. For instance, the Qwen-2.5-VL-7B model achieves faithfulness scores of only about 50 across various datasets and methods, which is still a lot from ideal (near 1.0). 

\noindent \textbf{FaithAct can improve faithfulness.} Second, the introduction of FaithAct consistently boosts faithfulness, showing improvements across three tested models. For instance, InternVL3-8B achieves a score of 57.35 $\pm$ 29.40 on RealWorldQA with FaithAct, compared to 44.23 $\pm$ 25.43 without it. Generally, our method achieves the best performance on 7 of 9 comparisons among all baselines. 

Notably, our results demonstrate a dramatic increase in performance on hallucination benchmarks, particularly on MMHal, where models incorporating FaithAct show a significant reduction in hallucinations. For instance, Qwen-2.5-VL-7B with FaithAct achieves a score of 66.45 $\pm$ 27.87, a notable improvement over its second best score of 56.77 $\pm$ 25.86. These results confirm that evidence-first reasoning, as enabled by FaithAct, significantly protects models from intermediate perceptual unfaithfulness while enhancing their overall faithfulness.


\subsection{Correctness Study}

Table~\ref{tab:correctness} shows\footnote{We evaluate the scores ourselves due to no official results provided in their technical report, serving as a baseline for future work.}

\subsection{Faithfulness Score Distribution}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/qwen.png}
    \caption{Distribution of $F_{step}$.}
    \label{fig:distribution}
\end{figure}

\subsection{Case Study}

Table~\ref{tab:correctness} shows\footnote{We evaluate the scores ourselves due to no official results provided in their technical report, serving as a baseline for future work.} the correctness score of Qwen-2.5-VL-7B with or without FaithAct on the three benchmarks we choose above. Our results demonstrate that with FaithAct, MLLMs can keep their capability on generating correct final answers to  the multimodal questions, and even a slight increase can be seen on this capability when evaluated on two of three benchmarks. Therefore, we can safely draw the conclusion that FaithAct can enhance the faithfulness of reasoning steps without doing harm to original reasoning correctness.


\subsection{Case Study}
We present qualitative comparisons on representative cases to illustrate how FaithAct improves perceptual grounding and reasoning consistency.

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figures/case_study_sichao.png}
    \caption{Qualitative comparison of reasoning chains generated with and without FaithAct on two illustrative cases. In both tasks, FaithAct enforces step-level perceptual verification, correcting hallucinated descriptions (top in red) and producing more structured, visually grounded reasoning (bottom in blue).}
    \label{fig:case_study}
\end{figure*}

We utilize Figure~\ref{fig:case} as an example. When the user query becomes ``\textit{What color is the bicycle and how many cars are visible (including thinking steps)?}'', the original model answer is:
\begin{tcolorbox}[notitle, boxrule=0pt,left=0.05cm, right=0.05cm, top=0cm, bottom=0cm]
\textit{1. The bicycle in the picture is \textcolor{red}{yellow}.}

\textit{2. There are \textcolor{red}{no cars} visible in the image, only a yellow bus and a person riding a bicycle.}

\textit{3. The bus appears to be ... \textcolor{red}{given its design and size}.}

\textit{4. The person on the bicycle is wearing a jacket and jeans.}
\end{tcolorbox} 
We \textcolor{red}{highlight} the nouns or phrases that represent perceptual unfaithfulness. After FaithAct, the reasoning process becomes:
\begin{tcolorbox}[notitle, boxrule=0pt,left=0.05cm, right=0.05cm, top=0cm, bottom=0cm]
1. Bus: The bus is yellow and is located on the right side of the image. It appears to be a public transport vehicle, likely a tram or trolleybus, given the context of the street scene.\textbackslash n\textbackslash n 2. Person: There is a person riding a bicycle. The person is wearing dark clothing and is positioned in front of the bus, indicating they are on the sidewalk.\textbackslash n\textbackslash n 3. Bicycle: The bicycle is \textcolor{ForestGreen}{white} and is being ridden by the person. It is located in the foreground of the image, close to the person.\textbackslash n\textbackslash n 4. Cars: There are \textcolor{ForestGreen}{two cars} visible in the image. One is behind the bus and the other may be at the edge of the image.\textbackslash n\textbackslash n Thus, there are two cars visible in the image.'
\end{tcolorbox} 

The results suggests that with FaithAct, perceptual unfaithfulness can be modified to a correct version by our MLLM with the guidance of evidence.



==> sec/intro.tex <==
\section{Introduction}

\subsection{\textcolor{red}{Motivation}}
We start the section by introducing the following principle.
\begin{quote}
    \textit{A perceptually faithful model reasons only over what is visually observable; it does not ``see'' what the image does not reveal.}
\end{quote}
\noindent This principle echoes long-standing findings in VQA: systems should avoid answering beyond available evidence and resist over-reliance on language priors \cite{goyal2017making,agrawal2018don}.

As illustrated in Figure~\ref{fig:motivation}, multimodal large language models (MLLMs) can produce seemingly correct answers and fluent explanations while exhibiting \textit{unfaithful} reasoning. We highlight two complementary failure modes. \textbf{Left:} a case of \emph{compound unfaithfulness} in which the model’s explanation is both \emph{behaviorally} unfaithful (a post-hoc narrative that does not reflect its decision process) and \emph{perceptually} unfaithful (claims about arrows/dots that do not match the input). \textbf{Right:} a case of \emph{behaviorally faithful but perceptually unfaithful} reasoning: the explanation traces the model's internal guess, yet asserts a color (``yellow bicycle'') that contradicts the image evidence. 

We therefore distangle \emph{behavioral faithfulness} (reasoning steps align with the model's decision) and \emph{perceptual faithfulness} (reasoning steps align with the input evidence) \cite{arcuschin2025chain, matton2025walk, ming2024faitheval,Li2023EvaluatingOH}. 
We argue that \textbf{faithfulness should be a design principle, not merely an evaluation objective}. Reasoning frameworks should \emph{explicitly verify} the evidential grounding of each step before it is admitted into the chain, ensuring that inference remains both perceptually justified and behaviorally aligned. This motivates \textsc{FaithAct}, a faithfulness-first planning framework that integrates evidence verification into every stage of reasoning, turning free-form chains of thought into \emph{chains of evidence}.

==> sec/methodology.tex <==
%\section{Methodology}

\section{Faithfulness in Current Reasoning}
\begin{comment}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/motivation.pdf}
    \caption{Motivation}
    \label{fig:motivation}
\end{figure}
\end{comment}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/motivation_sichao.png}
    \caption{Examples of perceptual and behavioral unfaithfulness. \textit{Left}: \textbf{Behavioral unfaithful and perceptual unfaithful.} The model presents a  step-by-step reasoning trace describing alternating arrow directions and increasing dot counts, yet such reasoning does not reflect its actual decision process. The final choice (A) is likely made through pattern association, with the explanation generated post hoc to rationalize it. \textit{Right}: \textbf{Behavioral faithful but perceptual unfaithful}. The model describes the bicycle as yellow, influenced by the nearby yellow bus, even though the bicycle is gray. This illustrates a visually plausible but perception-unfaithful reasoning step, where linguistic association overrides perceptual grounding.
}
    \label{fig:motivation}
\end{figure*}

As illustrated in Figure~\ref{fig:motivation}, reasoning chains often exhibit issues: the model’s intermediate thoughts introduce or rely on objects that are not actually in the input. For instance, when describing a street scene, MLLMs may refer to “bicycles” or “scooters” despite none being visible, producing seemingly logical but unsupported reasoning. Such inconsistencies reflect a gap between reasoning validity (internal logical soundness) and reasoning faithfulness (external evidential grounding). Faithfulness, in this context, measures whether every intermediate inference step is supported by the actual perceptual evidence rather than by statistical priors or linguistic biases. Existing reasoning frameworks, such as~\cite{ming2024faitheval, Li2023EvaluatingOH}, focus on improving correctness through step-by-step explanations, yet they rarely explore the issue above. Consequently, even well-structured reasoning traces can remain unfaithful. To address this limitation, we argue that future reasoning frameworks must explicitly incorporate evidence verification into each reasoning step, transforming reasoning chains into verifiable chains with evidence.



\section{Quantifying Reasoning Faithfulness Through Evidence Verification}
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/method-draft.pdf}
    \caption{Caption}
    \label{fig:placeholder}
\end{figure*}

\textcolor{red}{As illustrated in xxx, VLMs often hallucinate intermediate objects or claims not supported by the input image. Such ungrounded reasoning steps lead to unfaithful reasoning chains Prior work~\cite{li2023evaluating} also called this phenomenon \textit{object hallucinations} in vision tasks. } To systematically measure the faithfulness of reasoning steps, we propose a quantitative evaluation pipeline that verifies whether every claimed object is visually supported by the evidence. This Sec our extraction of claimed objects in Section~\ref{subsec:objectext}, and then two verification techniques to determine whether objects are really in the images in Section~\ref{subsec:grounding} and~\ref{subsec:poll}, finally faithfulness score judgement in Section~\ref{subsec:judge}. \textcolor{blue}{can add 2 python-style pseudo code here}

\subsection{Extraction of Claimed Objects}
\label{subsec:objectext}
\textcolor{red}{It's supposed to extract from both question and reasoning steps, right? Reasoning starts from the question to model, and the current opening misses the intro of setting. This could either here or above paragraph.}


To extract the claimed objects from the reasoning chain, we begin by leveraging MLLMs to reason step by step. Specifically, we employ a structured reasoning process where each step is independently processed, excluding introductory or concluding phrases such as “Let’s begin ...” and final answer statements. This allows us to isolate the core reasoning steps and focus solely on the intermediate claims made during the reasoning process. Each reasoning step is then parsed through a helper LLM for meaningful object extraction. A Qwen2.5-7B-Instruct~\cite{qwen2.5} is queried to return a set $O$ of $m$ objects \{$O_1, O_2, ..., O_{m}$\}. We place our prompt and some examples in Appendix~\ref{appendix:object_ext_prompt} to show the exactness of this step. This process ensures that only meaningful objects, such as physical items, concepts, or entities may occur in input images, are considered. 

\subsection{Technique: Grounding}
\label{subsec:grounding}
To verify whether the claimed objects in each reasoning step are present in the provided images, we employ a grounded object detection method using a frozen GroundingDINO-base model~\cite{liu2023grounding}. For each object \( O_t \) extracted from a reasoning step, GroundingDINO returns a set of bounding boxes \( B_t = \{b_{t}^1, b_{t}^2, ..., b_{t}^k\} \), where each bounding box \( b_{i}^k\) represents a region in the image that the model associates with the object \( O_t \). The model also provides a confidence score for each bounding box, denoted as \( C_{g_{t}} = \{c_{g_{t}}^1, c_{g_{t}}^2, ..., c_{g_{t}}^k\} \), indicating the probability that the object is indeed present in that bounding box. 

These bounding boxes and confidence scores are maintained in sets, with each object having its own set of bounding boxes and corresponding confidence scores. If multiple bounding boxes are returned for the same object, we retain the bounding boxes with the highest confidence scores to represent the most reliable detections. Thus, a set of confidence scores in each reasoning step can be kept as \( C_{g} = \{c_{g}^1, c_{g}^2, ..., c_{g}^m\} \), where $c_{g}^m=max(C_{g-m})$.

%This grounding step provides an essential function in our method, as it allows us to quantitatively assess whether the claimed objects in the reasoning chain align with the actual content of the image. The next step is to evaluate the reliability of the grounding process through a poll-based verification, as discussed in the following section.

\subsection{Technique: Preference Polling}
\label{subsec:poll}

While GroundingDINO is effective in localizing objects, it still suffers from limitations such as failure in grounding objects with weak visual salience or visual noise, empirically. To address these issues, we introduce a further verification function: \textit{Preference Polling}. \textcolor{blue}{TODO: need modification, confidence score unreliable, sometimes no detection, etc.}

The goal of this function is to quickly determine, for a given image and a claimed object, whether the object is truly present in the image, and to return both a binary existence label \{0,1\} and a corresponding confidence score. Concretely, we employ a frozen CLIP-VIT-large~\cite{radford2021learning} model as the vision-language encoder ($f_{img}, f_{txt}$), and append a lightweight polling head, a two-layer MLP with a hidden dimension of 512 and GELU activation, to perform the binary classification. The polling model is trained on POPE~\cite{Li2023EvaluatingOH}, a large-scale dataset with image-object existence labels. Training details are in Appendix~\ref{appendix:clip_training}.

Given an image \( I \) and an object text \( X \), the confidence score \( c_{p} \in [0, 1] \), interpreted as the probability that the object is present in the image, is as:
\begin{equation}
    \mathbf{v} = f_{img}(I) \in \mathbb{R}^{d}, \quad \mathbf{t} = f_{txt}(X) \in \mathbb{R}^{d},
\end{equation}
\begin{equation}
    c_{p} = \sigma \left( \mathbf{W}_2 \cdot \mathrm{GELU}(\mathbf{W}_1 (\mathbf{v} \odot \mathbf{t})) \right),
\end{equation}

where \( \mathbf{W}_1 \in \mathbb{R}^{512 \times d} \), \( \mathbf{W}_2 \in \mathbb{R}^{2 \times 512} \), and \( \sigma \) is the sigmoid function. By this way, a set of reliable confidence scores \( C_{p} = \{c_{p}^1, c_{p}^2, ..., c_{p}^m\} \) by polling can be maintained for each reasoning step.


\subsection{Faithfulness Score Judgment}
\label{subsec:judge}
On maintaining $C_g$ and $C_p$ for each step, we first consider both of them to define the overall confidence $c^t$ of an object $O_t$ in this step:
\begin{align}
    c^t = \alpha c_{p}^t + (1-\alpha) c_{g}^t, c_{p}^t \in C_{p},\nonumber \\ c_{g}^t \in C_{g}, \quad t \in \{1, 2, ..., m\},
\end{align}
since confidence scores from preference polling directly reflects whether an object exists or not, we set $\alpha$ to 0.7 empirically. Additionally, a threshold is set to represent whether object is in an image or not. We classify the overall confidence to three categories and define a mapping from confidence score to faithfulness score $f^t$ of the object: (1) $c^t < 0.4$, certain that $O_t$ does not exist, $f^t=0$; (2) $0.4< c^t < 0.6$, uncertain whether $O_t$ exists, $f^t=c^t$; (3) $c^t > 0.6$, certain that $O_t$ exists, $f^t=1$.

Based on this, we can define two scores for faithfulness, providing multi-level information. They are: (1) step-level faithfulness score $F_{step-i}$, depicting the faithfulness of each reasoning step (2) final faithfulness score $F_{chain}$, revealing the total faithfulness towards one reasoning chain. Note that we suppose n steps are in one chain (except excluding introductory or concluding steps). 
They are calculated as (suppose one reasoning process has $n$ steps):
\begin{equation}
    F_{step_{i}} = \frac{1}{m}\Sigma f^t,
\end{equation}
\begin{equation}
    F_{chain} = \frac{1}{n}\Sigma F_{step_{i}},
\end{equation}
This means if an MLLM generates more objects probably do not exist during reasoning, the faithfulness of reasoning process will be lower. Otherwise, the result will be different. 

\section{FaithAct: Faithfulness-First Planning}
The previous section established how reasoning faithfulness can be quantified by verifying whether each claimed object is visually supported. FaithAct extends this idea from evaluation to control: rather than verifying faithfulness after reasoning, it plans reasoning steps under explicit faithfulness constraints. The planner operates in a perception–planning–verification loop, ensuring that every reasoning action is grounded in observable evidence before proceeding to the next step.

Considering the measurement process, the further goal of our research is to enhance the faithfulness during the reasoning process of MLLMs. Thus, we propose a new planner for reasoning, Faithfulness-First Planner (FaithAct), to facilitate reliable reasoning process. The planner combines claimed object extraction, function calling in Section~\ref{subsec:calling} and refine-based reasoning in Section~\ref{subsec:refine}.

\subsection{Planning Objective}
We explicitly frame reasoning process as a faithfulness-constrained planning problem: Given a query and image, the planner seeks a sequence of reasoning actions:
\begin{equation}
    \pi^{*} = \arg \text{max} \mathcal{R}(\pi) \quad \text{s.t. } F_{step}(\pi_t) > c, \,\ \forall t,
\end{equation}
where $\pi_{t}$ is the $t$-th reasoning step, $F_{step}(\pi_t)$ is its faithfulness score from Section 4, and $c$ is a minimum evidential confidence threshold.
This converts reasoning into a faithfulness-regularized plan optimization: only steps sufficiently supported by evidence are eligible to advance the reasoning chain.

\begin{comment}
\subsection{OoI Extraction}
\label{subsec:ooi}
At the beginning of the reasoning process, the planner first queries the MLLM itself to generate a set of objects that it considers relevant and potentially helpful for the given task based on both image and text modality. These objects are defined as \textit{objects of interest} (OoI). Notably, we allow possible hallucinations at this stage. It means that the extracted objects may not necessarily exist in the input image. The rationale is that we aim to capture the model's own attention or semantic focus before imposing any faithfulness constraint.

However, through preliminary experiments, we observe that the MLLMs sometimes overly rely on visual bias, while sometimes ignoring important objects explicitly mentioned in the textual query. To mitigate this issue, we introduce a complementary extraction step based on the textual modality. Specifically, the MLLM is prompted again using the question text only, and generates another object set that reflects the textual semantics of the task.

Finally, the union of these two object sets is taken as the final set of OoI. This ensures that both visually and semantically important entities are covered. Prompts and some preliminary experiment results are in Appendix~\ref{appendix:ooi_prompts}.
\end{comment}

\subsection{Planning Loop}
\label{subsec:calling}

At each iteration, FaithAct performs three phases (as shown in Fig. x): 1. verify 2. ground 3. \textcolor{red}{plan The planner, a lightweight reasoning controller (an instruction-tuned MLLM)}, composes executable steps such as SELECT, ABSTAIN or COUNT, etc. using both textual input and verified visual states. Each planned step is validated by the faithfulness metrics before execution.

Detailedly, we utilize the functions to provide extra evidence information of the objects in reasoning steps for MLLMs. Here are them:
\begin{itemize}
    \item \texttt{Poll()}. When calling this, the function returns a direct probability of existence of an object based from polling model on Section~\ref{subsec:poll}.
    \item \texttt{Ground()}. Since location information is important for reasoning, we keep this technique from Section~\ref{subsec:grounding} as a function. When calling this, the function returns bounding boxes and confidence scores. 
    \item \texttt{Select()}. Based on Section~\ref{subsec:judge}, if the overall confidence of an object is higher than threshold, we select it as existence.
    \item \texttt{Abstain()}. Based on Section~\ref{subsec:judge}, if the overall confidence of an object is lower than threshold, we abstain it.
    \item \texttt{Count()}. Based on results from \texttt{Ground()}, this function counts the number of \textbf{reliable} bounding boxes and returns the number of the object.
\end{itemize}

Note that \texttt{COUNT} is a functional method (others mentioned here are verification methods). And we can add more functional methods like attribute, relate and so on, to build a detailed-yet-faithful reasoning chain.

\begin{algorithm}[t]
\caption{Faithfulness-First Planner (FaithAct)}
\label{algo:fplan}
\begin{algorithmic}[1]
\REQUIRE Image $I$, textual query $Q$, MLLM $M$, helper LLM $H_{M}$
\ENSURE Faithful reasoning output $R$

\STATE \textbf{// Step 1: Raw Reasoning}
\STATE $R_{raw} \gets M.\text{Reason}(I, Q)$ 
\STATE \textbf{//Step 2: Extraction of All Claimed Objects}
%\STATE $OoI_{img} \gets M.\text{ExtractOoI}(I, Q)$
%\STATE $OoI_{txt} \gets M.\text{ExtractOoI}(Q)$
%\STATE $OoI_{final} \gets OoI_{img} \cup OoI_{txt}$ 
%\STATE $R_{raw} \gets M.\text{Reason}(I, Q)$ 
\STATE $O_{raw} \gets H_{M}.\text{ExtractObj}(R_{raw})$
\STATE \textbf{// Step 3: Function Calls on Each Object}
\FOR{each object $o_i \in O_{raw}$}
    \STATE $c_{p}^i \gets \texttt{Poll}(o_i)$ \COMMENT{Existence confidence}
    \STATE $B_i, c_{g}^i \gets \texttt{Ground}(o_i)$ \COMMENT{Bounding boxes and scores}
    \STATE $ f^i \gets \texttt{SELECT}(c_{p}^i, c_{g}^i)$ or $\texttt{ABSTAIN}(c_{p}^i, c_{g}^i)$ \COMMENT{Higher than threshold, select the object; otherwise abstain.}
    \IF{\texttt{SELECT}}
    \STATE $n_i \gets \texttt{Count}(B_i, C_i)$ 
    \COMMENT{Number of detected instances}
    \STATE ...
    \ENDIF
\ENDFOR

\STATE \textbf{// Step 4: Refine-based Faithful Reasoning}
\STATE $R_{new} \gets M.\text{Reason}(I, Q, O_{raw}, \{f^i, B_i, n_i\})$

\STATE \RETURN $R_{new}$
\end{algorithmic}
\end{algorithm}

\subsection{Refine-based Reasoning}
\label{subsec:refine}

\paragraph{\textnormal{Thus, the whole reasoning process with FaithAct can be represented as Algorithm~\ref{algo:fplan}. This is a refine-based process. Firstly, the MLLMs are queried to provide a raw reasoning chain. Same as Section~\ref{subsec:objectext}, the helper LLM is used to extract claimed objects. We then call the functions to do faithful verification and provide extra information. These information helps the MLLM to refine the original reasoning process to be more faithful. We design special prompts to integrate the origin task problem with these extra information. Details can be seen in Appendix~\ref{appendix:f_plan_prompts}.}}

==> sec/related.tex <==
\section{Related Work}

\noindent \textbf{Faithfulness.} Considering the above problem, faithfulness in multimodal models are proposed to describe the degree to which generated explanations reflect the true evidence in the input (image, text, etc.), rather than relying on model biases or hallucinations. Several works have introduced benchmarks or metrics to evaluate faithfulness explicitly. M$^4$~\cite{li2023m4}, FaithScore~\cite{jing2023faithscore} and TIFA~\cite{hu2023tifa} propose metrics for evaluating the faithfulness for vision-language models. However, prior work seldom focus on the faithfulness of the reasoning chain, leaving an emergent research question here.

\noindent \textbf{MLLM Reasoning.}
MLLMs have developed surprising reasoning capabilities on multimodal problem solving, task planning, scientific discovery and so on~\cite{lumathvista, li2025chemvlm, gao2024cantor,an2024mc, an2025unictokens, lin2025perceive, li2025miv, li2025taco}. A famous research area of this topic is multimodal COT. Prior works like~\cite{chen2024m3cot, sun2025mm, shao2024visual, zhou2025logic, wang2025vl} apply multi reasoning steps to ensure the correctness of the final results. These methods can generate a long, detailed reasoning chain. However, MLLMs often generate some items not consistent with the visual information during reasoning~\cite{yu2024rlhf}. Thus, a mechanism to make the intermediate steps of reasoning process more reliable is crucial.

\noindent \textbf{Object Hallucination of MLLMs.}
Object hallucination refers to the tendency of MLLMs to mention or reason about objects that do not actually appear in the input images. This phenomenon reflects a mismatch between visual grounding and generated text, undermining the faithfulness and reliability of multimodal reasoning. To systematically evaluate this, several benchmarks have been developed. POPE~\cite{Li2023EvaluatingOH}, MMHal-Bench~\cite{sun2024aligning} are some of them.


